An Optimal Lower Bound for Buffer Management in Multi-Queue Switches

In the online packet buffering problem (also known as the unweighted FIFO variant of buffer management), we focus on a single network packet switching device with several input ports and one output port. This device forwards unit-size, unit-value packets from input ports to the output port. Buffers attached to input ports may accumulate incoming packets for later transmission; if they cannot accommodate all incoming packets, their excess is lost. A packet buffering algorithm has to choose from which buffers to transmit packets in order to minimize the number of lost packets and thus maximize the throughput. We present a tight lower bound of e/(e-1) ~ 1.582 on the competitive ratio of the throughput maximization, which holds even for fractional or randomized algorithms. This improves the previously best known lower bound of 1.4659 and matches the performance of the algorithm Random Schedule. Our result contradicts the claimed performance of the algorithm Random Permutation; we point out a flaw in its original analysis.

==> conclusions.tex <==
\section{Conclusions}

We conclude with a few remarks about the fractional model.
First of all, the buffer size $B$ does not seem to be a relevant factor, at
least for all known algorithms and lower bounds. Therefore, the fractional
model seems to be simpler than the standard, integral one and developing
optimal algorithms might be easier here.  

For the fractional model, we presented a new tight lower bound of $\e / (\e -
1)$, which matches the performance of the algorithm {\sc Frac-Waterlevel} by
Azar and Litichevskey~\cite{buffers-azar-litichevskey}.  Although optimal when
$m$~tends to infinity, the bound is not applicable for smaller values of $m$.
For $m = 2$, the exact competitive ratio of $16/13$ is achieved by the {\sc
Perpendicular Bisector} algorithm of~\cite{packet-buffering-two-optimal}; it
matches the lower bound generated by the uniform strategy
of~\cite{buffers-albers-schmidt}.  Determining the exact competitive ratios for
other values of $m$ is an open problem.  In particular, it is not even clear
whether the best possible lower bound can be incurred using canonical
strategies.



==> flaw.tex <==
\section{Flaw in the Analysis of the Random Permutation Algorithm}

The lower bound presented in this paper contradicts the claimed performance of
the {\sc Random Permutation} algorithm.  In this section, we demonstrate an error in
its original analysis~\cite{buffers-schmidt}. In terms of our lower bound, the
main source of the flawed analysis in~\cite{buffers-schmidt} is an assumption that
$\B$-uniform strategies are the worst for an online algorithm.

{\sc Random Permutation} is defined for $B = 1$ and any number $m$ of buffers.
It chooses a permutation of the buffers uniformly at random.  In any time step,
it transmits a packet from the populated buffer which is most to the front in
the permutation. 

The first packet arriving at a particular buffer is called {\em initializing}
and all the subsequent packets injected to this buffer are {\em
non-initializing}. We number all non-initializing packets.  The probability of
accepting the $i$-th non-initializing packet is denoted $p_i$. Let 
\[
	q_i = \frac{1}{m!} \cdot \sum_{j=1}^i \binom{i}{j} (m-j)! (-1)^{j-1} 
	\enspace.
\]
Lemma~1 of~\cite{buffers-schmidt} states that $p_i \geq q_i$ for $1 \leq i \leq m$, 
provided that $\OPT$ can accommodate all non-initializing packets.

In the proof of this lemma, it is argued that the worst possible situation occurs when
all $m$ initializing packets arrive at time 0 and then, for $1 \leq i \leq m$,
the $i$-th non-initializing packet arrives at time $i$ to buffer~$i$.  
We call such an input sequence {\em systematic} (these are inputs generated by special 
types of uniform strategies used in our construction).
Although the lemma holds for systematic sequences (it even holds that $p_i = q_i$), 
it is {\em not true} that the systematic sequences are the worst input instances for the {\sc Random
Permutation} algorithm.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
Our counterexample to Lemma 1 of~\cite{buffers-schmidt} is extremely simple.
Let $m = 10$; $m$ initializing packets are injected at time $0$.  For $1 \leq
i \leq 7$, the $i$-th non-initializing packet is injected at time~$i$ to buffer
$i$. At time $8$, no packets are injected.  At time $9$, $8$-th and $9$-th
non-initializing packets are injected to buffers~$8$ and~$9$, respectively. At
time $10$, the $10$-th non-initializing packet is injected to buffer $8$. 

Note that till step $7$, our sequence is systematic.  The probabilities of
accepting the $8$-th and the $9$-th packet are indeed slightly higher in our sequence
than in the systematic one, i.e., up till step $9$ claiming that the systematic
sequence is the worst possible is justified.  But our construction leaves
buffers $8$ and $9$ full at time~$9$.  Thus, the probability of accepting
the $10$-th non-initializing packet is at most $1/2 < q_{10}$. 
Note that this counterexample to the performance of {\sc Random Permutation}
follows the same line of attack as our lower bound, 
i.e., delaying the injections, filling multiple buffers at once, and 
finally injecting a subsequent packet to one of them.

Subsequent parts of the analysis of {\sc Random Permutation}~\cite{buffers-schmidt}
use only the relation $\sum_{k=1}^m p_k \geq \sum_{k=1}^m q_k$, which can be proved
to be false using our construction as well.
Showing it analytically would 
require tedious calculations and would be in a great part  
a mere repetition of the arguments given in the original proof of~\cite{buffers-schmidt}.
Since our construction is a small finite object, it can be verified by a
trivial computer program. Such program can be found on the author's web page. Here, 
we just list the relevant values. Clearly, $p_i = q_i$ for $i \leq 7$. 
Moreover $p_8 = p_9 = 2\,374\,894 / 10!$ and $p_{10} = 1\,716\,050 / 10!$, 
whereas $q_8 = 2\,012\,014 / 10!$, $q_9 = 2\,160\,343 / 10!$, and 
$q_{10} = 2\,293\,839 / 10!$. This shows that $\sum_{k=1}^m p_k < \sum_{k=1}^m q_k$,
proving Lemma~1~of~\cite{buffers-schmidt} false.



